Scalable and Interactive Electricity Grid Expansion Planning

Large scale grid expansion planning studies are essential to rapidly and efficiently decarbonizing the electricity sector. These studies help policy makers and grid participants understand which renewable generation, storage, and transmission assets should be built and where they will be most cost effective or have the highest emissions impact. However, these studies are often either too computationally expensive to run repeatedly or too coarsely modeled to give actionable decision information. In this study, we present an implicit gradient descent algorithm to solve expansion planning studies at scale, i.e., problems with many scenarios and large network models. Our algorithm is also interactive: given a base plan, planners can modify assumptions and data then quickly receive an updated plan. This allows the planner to study expansion outcomes for a wide variety of technology cost, weather, and electrification assumptions. We demonstrate the scalability of our tool, solving a case with over a hundred million variables. Then, we show that using warm starts can speed up subsequent runs by as much as 100x. We highlight how this can be used to quickly conduct storage cost uncertainty analysis.

==> v0.tex <==
We propose using the differentiable production cost modeling framework from~\cite{?degleris} and extending it to support warm starts.
The model is differentiated using the implicit function theorem, and the sensitivity of any outcome (such as emissions, prices, or generator schedules) can be computed with respect to any input (such as solar or transmission capacities).
Expansion planning problems are solved using gradient descent, i.e., by repeatedly simulating the grid and updating investments using the sensitivities, similar to how planners use sensitivities and prices to propose new upgrades in practice.
We extend the model to support warm starts, allowing planners to perturb parameters or assumptions (e.g., expected load or transmission upgrade costs) and obtain a modified plan in a short period of time.
Our framework is written in Python and supports large scale grid models (hundreds or thousands of nodes at an hourly resolution) with realistic grid constraints, e.g., (DC) linearized power flow, generator ramping, and battery storage.
